Word2Vec vs DBnary: Augmenting METEOR using Vector Representations or Lexical Resources?

This paper presents an approach combining lexico-semantic resources and distributed representations of words applied to the evaluation in machine translation (MT). This study is made through the enrichment of a well-known MT evaluation metric: METEOR. This metric enables an approximate match (synonymy or morphological similarity) between an automatic and a reference translation. Our experiments are made in the framework of the Metrics task of WMT 2014. We show that distributed representations are a good alternative to lexico-semantic resources for MT evaluation and they can even bring interesting additional information. The augmented versions of METEOR, using vector representations, are made available on our Github page.

==> conclusion.tex <==

In this article, we proposed to compare similarity measures between sentences based on representations distributed with similarity measures based on lexico-semantic networks.
More precisely, we proposed to extend the metric METEOR used for the evaluation of the automatic translation. 
In spite of the reserves which one can issue on the linguistic foundations of these distributed representations, we showed that they can be use when no lexico-semantic data are available.
Moreover, it seems these representations can bring a significant complement to the lexico-semantic data.
According to our experiments on English, German and Russian, the combination of these two types of information is promising for the automatic evaluation in automatic translation.
%  Moreover, the observations made on French are found on English, German and Russian.
The complementarity of the approaches seems to exist on several languages.


We consider to extend these techniques of pairing beyond word and to take into account a pairing on the level of the segment, even of the sentence.
We also plan to study the behavior of the distributed representations when one applies classical information retreival preprocessings like deleting empty words, for example.
Moreover, we will study the adaptation of these approaches on other metric automatics using of the lexical resources (e.g.: TER-Plus).
Lastly, we consider to use the distributed representations of words in other fields like confidence measure estimation.
For instance, in automatic translation, we would measure the existing correlations between the confidence measures enriched with post-editing times of translations.

The tool, the data and the models presented in this article are online\footnote{\url{http://anonymous-website.com}} to facilitate reproducibility of the experiments we carried out.
 


% Dans cet article, nous avons proposé de comparer les mesures de similarité entre phrases fondées sur des représentations distribuées avec des mesures de similarité fondées sur des réseaux lexicosémantiques.
% Plus précisément, nous avons proposé d’étendre la métrique METEOR utilisée pour l’évaluation de la traduction automatique. Malgré les réserves qu’on peut émettre sur les fondations linguistiques de ces représentations distribuées, nous avons montré qu’elles peuvent apporter un complément non-négligeable aux données lexico-sémantiques. 
% D’après nos expériences, l’association entre ces deux types d’information est prometteuse pour l’évaluation automatique en traduction automatique. 
% De plus, les observations faites sur le français se retrouvent sur l’anglais, l’allemand et le russe. 
% La complémentarité des approches semble donc exister sur plusieurs langues. 
% 
% Nous prévoyons d’étendre ces techniques d’appariement au-dela du mot et de prendre en compte un appariement au niveau du segment, voire de la phrase. 
% Nous envisageons également d’étudier le comportement des représentations distribuées lorsqu’on applique des pré-traitements classiques comme la suppresion des mots vides, par exemple. 
% De plus, nous étudierons l’adaptation de ces approches sur d’autres métriques automatiques utilisant des ressources lexicales (e.g. : TER-Plus). 
% Enfin, nous envigeons d’utiliser les représentations distribuées de mots dans d’autres domaines comme l’estimation de mesures de confiance. 
% Par exemple, en traduction automatique, nous souhaiterions mesurer les corrélations existantes entre des mesures de confiance enrichies avec des temps de post-édition de traductions.
% L’outil, les données et les modèles présentés dans cet article sont mis en ligne afin de faciliter la reproductibilité des expériences réalisées.
